Continual Hippocampus Segmentation with Transformers

In clinical settings, where acquisition conditions and patient populations change over time, continual learning is key for ensuring the safe use of deep neural networks. Yet most existing work focuses on convolutional architectures and image classification. Instead, radiologists prefer to work with segmentation models that outline specific regions-of-interest, for which Transformer-based architectures are gaining traction. The self-attention mechanism of Transformers could potentially mitigate catastrophic forgetting, opening the way for more robust medical image segmentation. In this work, we explore how recently-proposed Transformer mechanisms for semantic segmentation behave in sequential learning scenarios, and analyse how best to adapt continual learning strategies for this setting. Our evaluation on hippocampus segmentation shows that Transformer mechanisms mitigate catastrophic forgetting for medical image segmentation compared to purely convolutional architectures, and demonstrates that regularising ViT modules should be done with caution.

==> Content/01-Introduction_old.tex <==
While Continual Learning (CL) research often focuses on image classification benchmarks, recently its importance is realised in medical image segmentation. The application of deep learning methods for medical imaging tasks is strictly restrained, as time restrictions and privacy regulations both limit the access to data. However, the access to all data in such a setup is of utmost importance. CL solves this problem by gathering knowledge in a sequential training process extracted from a stream of datasets over a period of time \cite{gonzalez2020wrong, memmel2021adversarial}. Removing those limitations only shifts the problem to another area, as the evaluation of medical CL models has shown a significant drop in performance caused by the phenomenon called \textit{Catastrophic Forgetting}. This phenomenon occurs, as CL methods tend to strongly focus on the last trained task and thus forget previously learned knowledge \cite{kirkpatrick2017overcoming}. In medical imaging, the main reason of forgetting is the heterogeneity of medical data originated from multiple domains \cite{pianykh2020continuous}. 

The majority of CL methods is either focused on (1) convolutional based architectures or (2) regularisation based methods. Transformers \cite{vaswani2017attention, dosovitskiy2020image} however are promising for segmentation and CL due to their ability to handle sequential input data by using self-attention. In this article, we answer the question \textit{"Can the self-attention mechanism of Transformers be leveraged for continual medical image segmentation?"}. To address the utility of self-attention in retaining knowledge, we propose (1) a backbone model that combines state-of-the-art medical segmentation performance with Transformers as well as (2) an experimental setup to measure knowledge transferability over time. Additionally, we check (3) if popular regularisation based methods improve the performance when used in combination with Transformers.

The application of Transformers in medical imaging is not focused on continual segmentation and rather unexplored as recent work shows -- \cite{chen2021transunet, hatamizadeh2021unetr, karimi2021convolution, valanarasu2021medical, wang2021transbts}. Nevertheless, Transformer architectures are gaining traction in those fields as they may reduce forgetting due to their self-attention mechanism. In this work, \textit{we augment the state-of-the-art no-new-Net (nnU-Net) segmentation framework from Isensee} \etal~\cite{isensee2018nnu} \textit{with Transformer techniques} to leverage the self-attention mechanism for medical image segmentation. We further explore how the \textit{problem of Catastrophic Forgetting manifests in Transformer architectures} as opposed to pure convolutional layers. Last but not least, \textit{we adapt several popular CL methods for segmentation to analyse their performance when used in combination with Transformers} in a medical image segmentation setting. We conduct all experiments on the state-of-the-art nnU-Net so the experimental results do not suffer from low performance on the primary task of image segmentation. This setup is used to demonstrate the true potential of Transformers in medical imaging. We focus on continual hippocampus segmentation, as it is of utmost importance when it comes to diagnosing and selecting a promising treatment for neuropsychiatric disorders \cite{carmo2021hippocampus}. However, recent work has shown that hippocampus segmentation is very responsive to distribution shifts \cite{sanner2021reliable}. Our results show that self-attention can be leveraged to maintain knowledge in a CL setup, whereas regularising the attention mechanism has a negative effect and should be applied with caution.
